ML-based AIG Timing Prediction to Enhance Logic Optimization

As circuit designs become more intricate, obtaining accurate performance estimation in early stages, for effective design space exploration, becomes more time-consuming. Traditional logic optimization approaches often rely on proxy metrics to approximate post-mapping performance and area. However, these proxies do not always correlate well with actual post-mapping delay and area, resulting in suboptimal designs. To address this issue, we explore a ground-truth-based optimization flow that directly incorporates the exact post-mapping delay and area during optimization. While this approach improves design quality, it also significantly increases computational costs, particularly for large-scale designs. To overcome the runtime challenge, we apply machine learning models to predict post-mapping delay and area using the features extracted from AIGs. Our experimental results show that the model has high prediction accuracy with good generalization to unseen designs. Furthermore, the ML-enhanced logic optimization flow significantly reduces runtime while maintaining comparable performance and area outcomes.

==> sec/tbl-abc-commands.tex <==
\begin{table}
\centering
\caption{Transformation commands from ABC ~\blueHL{WJ: Jin, could you help to check if any documentation for what these commands trying to optimize and what are these options?}\redHL{JY: some of them are documented here:  https://people.eecs.berkeley.edu/~alanmi/abc/abc.rc Maybe we can just refer to this link and skip the table since some transformations are a customized sequence of a few commands}}
\label{tbl:abc-commands}
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{|c|c|c|} 
\hline
\textbf{Transformation} & \textbf{Option}    & \textbf{Comments}        \\ 
\hline
compress2rs             &                    &                          \\ 
\hline
dc2                     &                    &                          \\ 
\hline
resyn2                  &                    &                          \\ 
\hline
rewrite                 & -z, -l             &                          \\ 
\hline
drw                     &                    &                          \\ 
\hline
refactor                & -z, -l             &                          \\ 
\hline
resub                   & -z, -l, -M, -K, -N &                          \\ 
\hline
balance                 & -l                 & Reduce the level of AIG  \\ 
\hline
fraig                   &                    &                          \\
\hline
\end{tabular}
}
\end{table}
